Robust CAPTCHA Using Audio Illusions in the Era of Large Language Models: from Evaluation to Advances

CAPTCHAs are widely used by websites to block bots and spam by presenting challenges that are easy for humans but difficult for automated programs to solve. To improve accessibility, audio CAPTCHAs are designed to complement visual ones. However, the robustness of audio CAPTCHAs against advanced Large Audio Language Models (LALMs) and Automatic Speech Recognition (ASR) models remains unclear. In this paper, we introduce AI-CAPTCHA, a unified framework that offers (i) an evaluation framework, ACEval, which includes advanced LALM- and ASR-based solvers, and (ii) a novel audio CAPTCHA approach, IllusionAudio, leveraging audio illusions. Through extensive evaluations of seven widely deployed audio CAPTCHAs, we show that most existing methods can be solved with high success rates by advanced LALMs and ASR models, exposing critical security weaknesses. To address these vulnerabilities, we design a new audio CAPTCHA approach, IllusionAudio, which exploits perceptual illusion cues rooted in human auditory mechanisms. Extensive experiments demonstrate that our method defeats all tested LALM- and ASR-based attacks while achieving a 100% human pass rate, significantly outperforming existing audio CAPTCHA methods.

==> tables/RQ3.tex <==
\begin{table*}[t]
\centering
\caption{The pass rate of LALMs and ASR(-LLM)s on modern audio CAPTCHAs and sine-wave speech identification: LALMs under Zero-Shot and Chain-of-Thought prompting; ASR/ASR-LLM under Non-Prompt-Guide and Prompt-Guide.}
\label{tab:rq1_rq3_merged}
\resizebox{0.96\textwidth}{!}{%
\begin{tabular}{cc|cccccc|cccc}
\hline
\multicolumn{2}{c|}{\textbf{Method}} & \multicolumn{6}{c|}{\textbf{LALM}} & \multicolumn{4}{c}{\textbf{ASR/ASR-LLM}} \\ \hline
\multicolumn{2}{c|}{\textbf{Prompt-Mode}} &
\multicolumn{3}{c|}{\textbf{Zero-Shot}} &
\multicolumn{3}{c|}{\textbf{Chain-of-Thought}} &
\multicolumn{2}{c|}{\textbf{Non-Prompt-Guide}} &
\multicolumn{2}{c}{\textbf{Prompt-Guide}} \\ \hline
\multicolumn{2}{c|}{\textbf{Model-Name}} &
\multicolumn{1}{c|}{\textbf{Qwen}} &
\multicolumn{1}{c|}{\textbf{SeaLLMs}} &
\multicolumn{1}{c|}{\textbf{Qwen2}} &
\multicolumn{1}{c|}{\textbf{Qwen}} &
\multicolumn{1}{c|}{\textbf{SeaLLMs}} &
\textbf{Qwen2} &
\multicolumn{1}{c|}{\textbf{GPT4o-mini}} &
\multicolumn{1}{c|}{\textbf{GPT4o}} &
\multicolumn{1}{c|}{\textbf{GPT4o-mini}} &
\textbf{GPT4o} \\ \hline

% ---------------- Content-based Audio CAPTCHA ----------------
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\shortstack[c]{Content-based \\ Audio CAPTCHA}}}} &
\textbf{Geetest}   &
93.33\% & 96.66\% & \textbf{100.00\%} &
96.66\% & \textbf{100.00\%} & \textbf{100.00\%} &
\textbf{100.00\%} & \textbf{100.00\%} &
\textbf{100.00\%} & \textbf{100.00\%} \\
\multicolumn{1}{c|}{} &
\textbf{Google}    &
76.67\% & 80.00\% & \textbf{96.67\%} &
83.33\% & 80.00\% & \textbf{96.67\%} &
70.00\% & 80.00\% &
83.33\% & 80.00\% \\
\multicolumn{1}{c|}{} &
\textbf{MTCaptcha} &
\textbf{46.66\%} & 16.66\% & 30.00\% &
43.33\% & 13.33\% & 33.33\% &
10.00\% & 10.00\% &
16.66\% & 16.66\% \\
\multicolumn{1}{c|}{} &
\textbf{Telephone} &
6.67\% & 3.33\% & 6.67\% &
10.00\% & 3.33\% & 3.33\% &
10.00\% & 10.00\% &
20.00\% & \textbf{30.00\%} \\ \hline

% ---------------- Rule-based Audio CAPTCHA ----------------
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\shortstack[c]{Rule-based \\ Audio CAPTCHA}}}} &
\textbf{Math}      &
23.30\% & 0.00\% & 0.00\% &
\textbf{63.33\%} & 10.00\% & 3.33\% &
13.33\% & 20.00\% &
23.33\% & 23.33\% \\
\multicolumn{1}{c|}{} &
\textbf{Character} &
16.67\% & 16.67\% & 86.67\% &
26.67\% & 16.67\% & 86.67\% &
93.33\% & 93.33\% &
93.33\% & \textbf{96.66\%} \\
\multicolumn{1}{c|}{} &
\textbf{Arkoselabs} &
13.33\% & 3.33\% & 10.00\% &
\textbf{46.66\%} & 3.33\% & 6.66\% &
23.33\% & 23.33\% &
30.00\% & 30.00\% \\ \hline

% ---------------- Sine-wave speech identification ----------------
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\shortstack[c]{Sine-wave \\ Speech}}}} &
\textbf{Sine-Wave} &
0.00\% & 0.00\% & 0.00\% &
0.00\% & 0.00\% & 0.00\% &
0.00\% & 0.00\% &
0.00\% & 0.00\% \\
\multicolumn{1}{c|}{} &
\textbf{Diff-Sine-Wave} &
0.00\% & 0.00\% & 0.00\% &
0.00\% & 0.00\% & 0.00\% &
0.00\% & 0.00\% &
0.00\% & 0.00\% \\ \hline

\end{tabular}%
}
\end{table*}


==> tables/RQ5.tex <==
\begin{table*}[t]
\centering
\caption{The security and usability of AICAPTCHA:  `Best@AI' refers to the highest effectiveness of AI systems in identifying audio CAPTCHAs, while `F-Attempt@Human' indicates the success rate of human users on their first attempt.}
\label{tab:rq5}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{c|cccc|ccc|c}
\hline
\textbf{CAPTCHA-Type} & \multicolumn{4}{c|}{\textbf{Content-based Audio CAPTCHA}}      & \multicolumn{3}{c|}{\textbf{Rule-based Audio CAPTCHA}} & \textbf{Our Method} \\ \hline
\textbf{CAPTCHA-Name} & \textbf{GeeCAPTCHA} & \textbf{Google}  & \textbf{MTCAPTCHA} & \textbf{Telephone} & \textbf{Math}       & \textbf{Character}   & \textbf{Arkoselabs}   & \textbf{AICAPTCHA}  \\ \hline
\textbf{Best@AI}      & 100.00\%      & 96.67\% & 46.66\%   & 30.00\%         & 63.33\%    & 96.66\%     & 46.66\%      & \textbf{0.00\%}        \\
\textbf{F-Attempt@Human}   & \textbf{100.00\%}      & 23.33\% & 80.00\%      & 23.33\%      & 80.00\%       & 50.00\%     & 76.67\%      & \textbf{100.00\%}      \\ \hline
\end{tabular}%
}
\end{table*}

